Large-scale Evaluation of Notebook Checkpointing with AI Agents

Saving, or checkpointing, intermediate results during interactive data exploration can potentially boost user productivity. However, existing studies on this topic are limited, as they primarily rely on small-scale experiments with human participants - a fundamental constraint of human subject studies. To address this limitation, we employ AI agents to simulate a large number of complex data exploration scenarios, including revisiting past states and branching into new exploration paths. This strategy enables us to accurately assess the impact of checkpointing while closely mimicking the behavior of real-world data practitioners. Our evaluation results, involving more than 1,000 exploration paths and 2,848 executed code blocks, show that a checkpointing framework for computational notebooks can indeed enhance productivity by minimizing unnecessary code re-executions and redundant variables or code.

==> plots/fig/complexity_code.tex <==
% \documentclass[tikz,border=10pt]{standalone}
% \usepackage{pgfplots}
% \usepackage{pgfplotstable}

% \begin{document}
\begin{figure*}[t]
\begin{tikzpicture}
\begin{axis}[
    ybar,
    width=15cm,    
    height=40mm, 
    bar width=0.2cm,
    ymin=0,
    ymax=500,
    symbolic x coords={ 1, 2, 3, 4, 5, 6, 7, 8, 9, 10},
    xtick=data,
    ylabel={Peak number of cells},
    xlabel={Exploration session ID (each session explored 100 branches)},
    enlarge x limits=0.05,
    xlabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    every tick label/.append style={font=\footnotesize},
    area legend,
    legend style={
        at={(0.5,0.97)},
        anchor=north,
        legend columns=-1,
        /tikz/every even column/.append style={column sep=3mm},
        nodes={scale=0.75, transform shape},
    },
    nodes near coords,
    nodes near coords style={font=\footnotesize, text=black},
    tick align=inside,
    ymajorgrids
]

% Load the data from the file and plot it using \addplot+
\addplot+[ybar, fill=cBmain, draw=black] 
    table[x=group_number, y=naive_start_over, col sep=tab, header=true] {data/complexity_code.txt};

\addplot+[ybar, fill=cCmain, draw=black, pattern color=cClight, postaction={pattern=north west lines}] 
    table[x=group_number, y=naive_start_middle, col sep=tab, header=true] {data/complexity_code.txt};

\addplot+[ybar, fill=cAmain, draw=black] 
    table[x=group_number, y=Kishuboard, col sep=tab, header=true] {data/complexity_code.txt};

\legend{\nrestart,\ncontinue, \system}

\end{axis}
\end{tikzpicture}
\caption{\fix{The peak number of cells in the notebook for each session during exploration. 
Smaller numbers of cells may be preferred due to easier understanding
    of ongoing exploration.
\ncontinue creates excessive cells due to mixing all branches into one notebook.
\system does not create any unnecessary cells as it relies on
    checkpointing.}}
%don't say it's capped.worst case...

\vspace{-2mm}
\label{fig:complexity_code}
\end{figure*}

% Add the node outside the axis environmen

% \end{document}


==> plots/fig/complexity_var.tex <==
% \documentclass[tikz,border=10pt]{standalone}
% \usepackage{pgfplots}
% \usepackage{pgfplotstable}

% \begin{document}
\begin{figure*}[t]
\includegraphics[width=0.9\linewidth]{vector_figures/lbwfig4.pdf}
\caption{\fix{The peak number of kernel variables for each session during exploration. 
Smaller numbers of variables may be preferred for easier understanding.
\ncontinue produces excessive variables, increasing cognitive load to keep track of variables across branches. \system has exactly two more variables than \nrestart for user-invisible metadata.}}
%don't say it's capped.worst case...

\vspace{-2mm}
\label{fig:complexity_var}
\end{figure*}

% \end{document}


==> plots/fig/fig_user_interface.tex <==
\begin{figure*}[t]
\includegraphics[width=0.9\linewidth]{vector_figures/lbwfig1.pdf}
\vspace{-2mm}
\caption{
Background about \system.
The history graph (purple box) shows past commits.
The code and variable panes (yellow box) display
    the information of a selected commit.
From any past commit,
    users can load data only (i.e., execution rollback)
        or load both code and data (i.e., checkout)
    using the navigation popup (red box).
The image is reproduced with the original authors' permission.
}
\Description{
 This figure shows Kishuboard User Interface

The interface includes:

Search Bar: Filters commits based on keywords.
History Graph: Displays past commits with code and data states.
Navigation Popup: Allows switching between code+data states (rollback or checkout).
Code View & Variable Panel: Shows details of the selected commit without changing the active Jupyter session.
This interface helps users manage and explore different versions of computational notebooks effectively.
}
\label{fig:ui:kishuboard}
\end{figure*}

% \begin{figure*}[t]
% \input{plots/screenshot}
%     % \includegraphics[width=\linewidth]{figures/opening_figure.png}
%     \vspace{-2mm}
%     \caption{\hanxi{take another screenshot to show notebook cells and update the caption here. Also, update color palette for the highlights. Make the colors global variables in main} Our prototype UI for supporting two-dimensional checkout in the “code+data” space. 1: The code view shows the execution history and code cells for the selected commit.  2: The history graph shows the history of global branched exploration. (\cref{sec:version-viz}) 3: The search bar to search a specific commit. (\cref{sec:others_search}) 4: The variable pane for the selected commit. (\cref{sec:design-ui}) 5: An illustration of roll back execution operation to a history commit; the operation will keep the code and rollback only the data to the target commit.(\cref{sec:version-property}) Our design is based on formative interviews (\cref{sec:interview}) and mathematical principles (\cref{sec:version}). Our approach led to higher productivity (\cref{sec:productivity}) and positive responses (\cref{sec:ui_easiness}, \cref{sec:qualitative}) in user studies.}
%     \label{fig:ui:kishuboard}
% \end{figure*}


==> plots/fig/llm_e2e_time.tex <==

\begin{figure*}[ht]
\centering
\includegraphics[width=0.9\linewidth]{vector_figures/lbwfig3.pdf}
\caption{\fix{End-to-end execution time for \system and baseline methods. We generated \textbf{1000} branches of code using LLM-Agent, divided into 10 exploration sessions with 100 branches each. The sessions are sorted in ascending order by \nrestart time. \ncontinue method is the fastest in terms of execution time, as it only runs newly added cells without checkpoint or checkout overhead. However, it is faulty, often producing incorrect results that do not trigger explicit errors, which may require significant debugging time. The additional time for the \system group is due entirely to checkpointing and checkout overhead, with the worst-case average overhead being just 2 seconds per branch. The red annotations indicate the number of implicit incorrect results for each session.}}
%don't say it's capped.worst case....

\vspace{-2mm}
\label{fig:e2e_time}
\end{figure*}
%number of incorrect result
% average e2e, from 0.
%expand x label, each group ...
% bald error in caption
% another figure for example
% Add the node outside the axis environmen
% exploration session
% we generated 1000 in total, mention it in caption;


==> plots/fig/llm_example.tex <==
\begin{figure*}[t]
\includegraphics[width=0.9\linewidth]{vector_figures/lbwfig2.pdf}
    \caption{\fix{A toy example of user's intended data exploration and strategies to execute it. \nrestart repetitively executes cells $c_1$ and $c_2$. \ncontinue executes new cells ($c_{3'}$ and $c_{4'}$) without any kernel restart. \ncontinue may lead to branch interferences, for example, N/A values were already dropped by $c_3$, making data imputation in $c_{3'}$ ineffective. 
    \system restores checkpointed data to explore a new path,
        thus removing the repetitive work and preventing potential branch interferences.}}
    \label{fig:llm_group_example}
\end{figure*}

% \begin{figure*}[htbp]
%     \centering
%     \begin{subfigure}[b]{0.6\textwidth}
%         \centering
%             \begin{subfigure}[b]{\textwidth}
%         \centering
%     \includegraphics[width=\textwidth]{figures/nrestart.png}
%         \caption{\nrestart, a new notebook is started for the new branch}
%         \label{fig:subfig1}
%     \end{subfigure}

%         \begin{subfigure}[b]{\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/llm_kishuboard.png}
%         \caption{\system. Only one notebook is used for both branches.}
%         \label{fig:subfig3}
%     \end{subfigure}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.35\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/ncontinue.png}
%         \caption{\ncontinue, only one notebook is used for both branches. Note that the logic of cell 4 "process data" is now applied to both branches instead of only branch 1, causing error.}
%     \label{fig:naive_continue_example}
%     \end{subfigure}
%     \caption{\fix{Example of the three strategies for exploring two branches. Cell 1 and cell 2 are the same for both branches. \nrestart starts a new notebook and a new kernel for each branch; \system checkout the notebook and kernel state to start a new branch; \ncontinue appends the cells of the new branch (cell 6 and cell 7) to the current notebook and continue execution with the current kernel.}}
%     \label{fig:llm_group_example}
% \end{figure*}


==> sections/Conclusion.tex <==
\section{Conclusion}
In this study, we demonstrate the efficacy of using AI agents to evaluate notebook checkpointing systems at scale, addressing limitations inherent in traditional human-subject studies. Traditional user studies are constrained by limited participant pools, short durations, and the substantial costs of ensuring uniform skill validation, which collectively hinder the scale and diversity of such evaluations. In contrast, AI agents offer a scalable alternative by generating diverse code in a short amount of time, mimicking real-world exploratory behaviors, and producing high-quality code. By simulating diverse and complex data exploration scenarios—encompassing a total of 1,000 branches— we assessed the performance of Kishuboard, a novel code+data checkpointing framework, against baselines. The results show that Kishuboard significantly enhances exploration efficiency, reduces cognitive burden, and prevents branching errors. Our work is the first of its kind to demonstrate the utility of AI agents in evaluating notebook checkpointing systems.

==> sections/Exp_design.tex <==
\input{Source/plots/fig/llm_example}

\section{AI-Agent-Based Experiment Design}
\label{sec:design}
We tackle the limitations mentioned in \cref{sec:existing_eval} 
    using AI agents.
    As AI agents can generate diverse code
        in a short amount of time, compared to humans, 
    it allows us to evaluate \system's effectiveness 
        at a much larger scale
        in terms of code diversity at a relatively small cost.
    We first describe our experiment design in this section.
    Then, we examine its scientific validity in \cref{sec:validation}.
    
    \paragraph{Simulating Branched Data Exploration} We use a large language model (LLM),
        i.e., ChatGPT-4o~\cite{achiam2023gpt}, 
    to iteratively generate code cells based on a generic task specification. We first provide the task: ``My data is in \texttt{file\_name}. The columns and their meanings are \texttt{column\_names\_and\_descriptions}. I want to build a model to predict \texttt{requirements}.'' then prompt the LLM to outline a step-by-step plan. Afterward, we prompt the agent to generate code cells and execute the generated code according to the plan step by step. Specifically, the execution results and code for previous steps are fed to the agent when generating the code for next step. 

    % \paragraph{Simulating Branched Data Exploration}
    Data scientists often revisit previous explored phases~\cite{liu2019understanding,kery2018story,guo2013workflow,raghunandan2023code,koop2017dataflow,hohman2020understanding}. To simulate such a behavior, we randomly select a past cell to revisit and ask the LLM to generate alternative code cells to continue from the selected cell. Each time creates a new branch of exploration. Whenever a runtime error occurs, the LLM can retry twice to self-correct according to the error message. If the LLM fails to fix the error, we checkout randomly and start a new branch.
    \cref{sec:appendix:prompts} presents concrete examples
        of our prompts and generated code by the LLM.
    
    % \paragraph{Reiterating to Create a Large-scale Workflow}
    We repeat the generation process 10 times to simulate \textbf{10 exploration sessions} of data scientists exploring data independently where each session explores \textbf{100 branches}. The dataset is the 32~KB Titanic dataset downloaded from Kaggle~\cite{titanicdata}. Overall, the LLM generated \textbf{2,848} cells in this study. 

    To test \system's performance with memory-intensive tasks, we also use the Spotify podcast dataset (i.e., 45 MB and 450 MB)~\cite{spotifydata} to simulate 3 exploration sessions with each exploring 3 branches.
    
    \paragraph{Baselines and \system}
    Given an exploration session, we test the following existing baseline strategies and \system to support branched data exploration (see \Cref{fig:llm_group_example} for an example).
    (1) \textbf{\nrestart}: To explore a new branch, \nrestart restarts the kernel and re-executes common cells to restore the selected past state. This strategy follows some user's behaviour of starting a new notebook for a new exploration path~\cite{chattopadhyay2020s}.
    (2) \textbf{\ncontinue}: Instead, \ncontinue appends new cells to the current notebook and continues execution from the current kernel state
        without any restart. 
    It mimics a common practice to mix code from different cells within the same notebook~\cite{liu2019understanding,subramanian2019supporting,kery2018story}. \ncontinue can introduce both explicit errors (e.g., operating on columns dropped in an earlier branch, thus observing execution errors) or implicit errors (e.g., unknowingly working on a dataframe updated by an earlier branch).
    (3) \textbf{\system}: This approach leverages \system to check out the code+data version to the latest common history state and continue execution from there.

    \paragraph{Metrics}

    In addition to performance metrics (i.e., execution times), this experiment is also interested in measuring correctness and exploration complexity using the following metrics.
    (1) \textbf{End-to-end time to explore all branches}: This metric measures the time elapsed to execute and checkpoint/checkout code for all the generated branches.
    % Since each exploration session has 100 branches, this number equals the end-to-end time to explore all branches divided by 100, excluding the time spent on code generation or human factors such as browsing and writing code.
    It focuses solely on system efficiency during execution and state management (if any) as the time for AI-agents to generate code is neglected.
    (2) \textbf{Number of branch interferences}:
    % This metric tracks errors during code execution, including runtime errors (which prevent the code from running) and logical errors (which occur when variables are incorrectly accessed across branches). Since LLM's runtime errors are prevented by restarting branches upon failure during code generation, all errors are related to cross-branch interference.
    In the real world, a \emph{branch interference} occurs when a user reuses a modified variable assuming it was unmodified. Unfortunately, it may lead to misleading exploration outcomes which are hard to detect and debug.
    To study this type of mistake, we count the number of times a variable is incorrectly accessed across branches.
    % For example, if an earlier branch $B_1$ modifies a variable and a later branch $B_2$ accesses the modified variables, it results in a branch interference.
    For example, in \cref{fig:llm_group_example}, cell $c_3$ from the first branch drops rows with missing values in \texttt{df}, but with naively continue executing, cell $c_{3'}$ would ineffectively impute missing-but-already-dropped values which is a branch interference.
    We detect such branch interference by analyzing variable access and modification in each cell as well as manually verifying each detected branch interference.
    (3) \textbf{Peak number of variables}: This metric tracks the maximum number of variables in the kernel's namespace. A higher number indicates a greater memory burden and increased cognitive overhead for the user to remember and manage the variables.
    (4) \textbf{Peak number of cells}: This metric tracks the maximum number of cells in the notebook at any given time. A larger number of cells indicates a messier notebook cell organization, leading to difficulties working with the notebook and cognitive burden.


==> sections/Exp_results.tex <==

   \section{Experiment Result and Discussion}
    \label{sec:llm-result}

    Using the AI-agent-based methodology described earlier, we present and discuss the experiment results in this section in terms of correctness, efficiency, and notebook simplicity. In summary, we get the following experiment results:
     \begin{enumerate}
        \item \system speeds up data exploration: up to $36\%$ faster in both compute-intensive/light tasks, than naively restarting and re-execution. On average, data exploration with \system is $23\%$ faster in compute-intensive tasks and 
        $15\%$ faster in compute-light tasks
            in terms of execution times. 
        % Wherein, \system consumes at most 2.03 seconds per data exploration branch. 
        \item \system prevents incorrect results 
            that often occur when users na\"ively explore alternative paths
                by appending cells and/or reusing variables.
        \item \system maintains a clean notebook with only cells and variables in the current branch, which is 
            significantly more effective than
            keeping track of branched structures with (almost) redundant code and variables.
            % alleviating the user's burden to keep track of the branched structure of both code and variables.
        % \item For memory-intensive tasks, \system's overhead remains under 20\%.
        \item \system's space overhead---checkpoint sizes---is
            small.
        % accelerates data exploration in both memory-light and memory-intensive scenarios with relatively small checkpoint size.
    \end{enumerate}
    
    \paragraph{\system Speeds up Data Exploration} 
    We compare end-to-end times to explore using different strategies. \Cref{fig:e2e_time} shows that \system enables faster data explorations than \nrestart does. In Session 10, \system would save the user about 10 minutes of real-time or 36\% faster than \nrestart. As the only exception, \system is slightly slower than \nrestart in Session 2 because cells before the branching point are all lightweight, making recomputation faster than using recovering from checkpoints.
    \ncontinue is expectedly faster than \system as \ncontinue overwrites the existing kernel state by running only the additional cells (for a new exploration path);
    however, \ncontinue causes significant issues 
        such as branch interferences and incorrect results as described below.
    % which may take a longer time to debug. 

    \input{Source/plots/fig/complexity_var}
    % \input{plots/fig/complexity_code}
    
    \paragraph{\system Ensures Correctness} Furthermore, \system guarantees correctness (\Cref{fig:e2e_time}) by recovering exact data states from checkpoints.
    In contrast, while the alternative method \ncontinue is the fastest, it is error-prone. In particular, we detect 355 branch interferences which are hard to detect and debug manually.
    For example, in Session 9, Branch 5 modifies a variable \texttt{X\_test} by resampling from the original dataset and re-assigning it to the same variable name. Later on, Branch 7 evaluates its model based on \texttt{X\_test} which leads to a misleading accuracy because the resampled \texttt{X\_test} overlaps with the training data. 
    % \supawit{please read the example and feel free to revise it.} Good find, Hanxi!
    Unsurprisingly, \nrestart also guarantees correctness but incurs computation costs to re-execute cells common across branches.
    % Additionally, having only one kernel state means that switching branches requires re-execution, further complicating the debugging process.
    % On the other hand, \system ensures correctness by checking out kernel states for each branch, avoiding these issues while still being relatively efficient.

    \paragraph{\system Maintains Clean Code and Data States} To assess notebook complexity, we measure the peak number of variables during exploration, as shown in \Cref{fig:complexity_var}. Compared to \nrestart and \system, \ncontinue results in significantly more variables, 
    because \ncontinue mixes data states from multiple exploration branches. We also measure the peak number of cells in the notebook during exploration and find that the \ncontinue sessions have at least $24\times$ more cells than the other two groups, as it appends code from different branches to the same notebook.
    Consequently, the user of \ncontinue would experience an increased cognitive load to manage code cells across branches and remember variables.

% \begin{table}[ht]
% \centering
% \begin{tabular}{ccccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset Size}} & \multirow{2}{*}{\textbf{\nrestart e2e time}}& \multicolumn{3}{c}{\textbf{\system}} \\
% \cline{3-5}
%                         & & \textbf{e2e time} & \textbf{speed up} & \textbf{storage size}                         \\
% \hline
% 45MB                         & 38s    & 24s & 37\% & 56MB                      \\
% 450MB                         & 217s     & 169s & 22\% &  358MB                    \\
% \hline
% \end{tabular}
% \label{table:large_dataset}
% \caption{\fix{Performance of \system on small and large datasets with three randomly generated branches. The checkpoint storage size for \is 56MB ()Compared to \nrestart, \system achieves faster inference times for both small and large datasets, with the same code used for both. }}
% \end{table}
    
    \paragraph{Simulating Memory-intensive Tasks} Using the AI agent to explore both 45~MB and 450~MB Spotify dataset~\cite{spotifydata},
    our results presented in \cref{table:large_dataset} show that
    % by using incremental checkpoint technique~\cite{kishu},
    \system can checkpoint variables efficiently without requiring extensive IO overhead or storage resources. For the 45~MB dataset, the total checkpoint size was 56~MB, and for the 450~MB dataset, it was 358~MB---smaller than the dataset itself in a CSV format.
    % This reduction is because the original dataset is stored in CSV format, which is inefficient, whereas the checkpoints are saved as pickled pandas DataFrames, resulting in smaller sizes.
    Furthermore, \system accelerates data exploration in both memory-light and memory-intensive scenarios, demonstrating the scalability of the method.

    We observed that during experiments with larger datasets, \system occasionally fails with ``\texttt{OverflowError: BLOB longer than INT\_MAX bytes}'' due to a limitation in the existing backend implementation~\cite{kishu}.
    Because this issue is an implementation flaw and not inherent to the technique, we believe that it could be addressed by chunking data before writing to storage.

% \begin{table}[ht]
% \centering
% \begin{tabular}{ccccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset Size}} & \multirow{2}{*}{\textbf{\nrestart e2e time}} & \multirow{2}{*}{\textbf{\ncontinue e2e time}}& \multicolumn{2}{c}{\textbf{\system}} \\
% \cline{4-5}
%                         & & & \textbf{e2e time} & \textbf{storage size}                         \\
% \hline
% 45MB                         & 38s   & 18s   & 24s & 56MB                      \\
% 450MB                         & 217s   & 141s   & 169s &  358MB                    \\
% \hline
% \end{tabular}
% \caption{Grouped Table with Multiline Header}
% \end{table}
% \begin{table}[ht]
% \centering
% \begin{tabular}{ccccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset Size}} & \multirow{2}{*}{\textbf{\nrestart e2e time}} & \multirow{2}{*}{\textbf{\ncontinue e2e time}}& \multicolumn{2}{c}{\textbf{\system}} \\
% \cline{4-5}
%                         & & & \textbf{e2e time} & \textbf{storage size}                         \\
% \hline
% 45MB                         & 38s   & 18s   & 24s & 56MB                      \\
% 450MB                         & 217s   & 141s   & 169s &  358MB                    \\
% \hline
% \end{tabular}
% \caption{(another option for table 5.) Grouped Table with Multiline Header}
% \end{table}

% \begin{table}[ht]
% \centering
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{2}{*}{\textbf{Dataset size}} & \multicolumn{3}{c|}{\nrestart} & \multicolumn{4}{c|}{\ncontinue}& \multicolumn{4}{c}{\system} \\
% \cline{2-12}
%                           & \textbf{e2e time} & \textbf{\#cells} & \textbf{\#var} & \textbf{e2e time} & \textbf{\#cells} & \textbf{\#var} & \textbf{\#errors} & \textbf{e2e time} & \textbf{\#cells} & \textbf{\#var} &\textbf{checkpoint storage}                         \\
% \hline
% 45MB                        & 38 & 9 & 63 & 18 & 14 & 69 & 0 & 24 & 9 & 65 &56MB                       \\
% 450MB                        & 271 & 9 & 63 & 141 & 14 & 69 & 0 & 169 & 9 & 65 &358MB                     \\
% \hline
% \end{tabular}
% \caption{(another option for table 5.) Grouped Table with Multiline Header}
% \end{table}


\begin{table*}[t]
\caption{\fix{End-to-end execution time for exploring three randomly generated branches on small (45 MB) and large (450 MB) datasets. ``Time'' denotes the duration from executing the first cell of the first branch to completing the last cell of the final branch. ``\# of Cells'' and ``\# of Variables'' indicate the \textbf{peak} number of cells in the notebook and the peak number of variables in the kernel, respectively. 
\system outperforms \nrestart in efficiency for both dataset sizes, demonstrating the scalability of the method. Additionally, \system requires only 56 MB of storage for checkpoints on the small dataset and 358 MB on the large dataset throughout the exploration.
While \ncontinue is faster than \system, 
    as observed in the previous experiments,
    \ncontinue often causes hard-to-detect errors (\cref{fig:e2e_time})
        and creates significantly more variables(\cref{fig:complexity_var}) and cells.
}}
\label{table:large_dataset}
% \caption{\fix{\hanxi{Table description here: what is ``Time'', \#Cells, and \#Variables + \system's storage sizes + \system remains faster than \nrestart + \ncontinue may cause wrong results}}}

\centering
\small
\begin{tabular}{lrrrrrr}
\toprule
\multirow{2}{*}{\textbf{Method}}
    & \multicolumn{3}{c}{Small Dataset (45 MB)} & \multicolumn{3}{c}{Large Dataset (450 MB)}\\
% \cline{2-7}
    & \textbf{Time (secs)} & \textbf{\# of Cells} & \textbf{\# of Variables}  & \textbf{Time (secs)} & \textbf{\# of Cells} & \textbf{\# of Variables} \\
\midrule
\nrestart & 38 & 9 & 63 & 271 & 9 & 63 \\
\ncontinue & 18 & 14 & 69 & 141 & 14 & 69 \\
\system & 24 & 9 & 65 & 169 & 9 & 65 \\
\bottomrule
\end{tabular}
\end{table*}

==> sections/Limitations.tex <==
\section{Limitations of Experiment Setup and Result}
While our AI-agent-based evaluation provides a large-scale and systematic analysis of notebook checkpointing, several limitations must be acknowledged. These primarily stem from the differences in behavior between AI agents and human practitioners.

\paragraph{AI Agents Do Not Replicate How Humans Iteratively Explore Branches} The simulation of 100 randomly generated branches within a 10-cell notebook may not fully capture real-world data science workflows. While AI agents randomly revert to past commits, human users make such decisions based on logical reasoning or execution results. Furthermore, human users vary in exploration depth, leading to different numbers of executed cells per branch. This discrepancy may influence our findings, particularly in assessing the efficiency of different checkpointing strategies. For example, 
if humans always choose to checkout to a very
early stage, then the efficiency gap between \nrestart and \system may be smaller.

\paragraph{Unlike AI Agents, Humans Can Mitigate Variable Overwrites} The drawbacks observed in the \ncontinue group may not be as severe in real-world scenarios. Experienced users often mitigate variable overwrites by explicitly renaming or copying variables when switching between branches. As a result, the frequency of branch interferences leading to execution errors may be lower than what our AI-agent simulations suggest. Moreover, while AI agents append all executed cells into a single notebook, real users often refactor their workflow by removing obsolete cells or reorganizing their notebooks dynamically. However, it is important to note that these manual interventions take time—time that \system aims to save by automating refactoring and state management.

\paragraph{AI Agents Do Not Experience Cognitive Load} In real-world scenarios, users must actively navigate commit histories and decide which version to restore using \system. Similarly, those in the \ncontinue and \nrestart groups would spend additional time figuring out how to organize cells or new notebooks. These interactions, which require human judgment and effort, are not fully accounted for in our AI-driven evaluation.

Given these factors, while our AI-agent-based approach offers valuable insights into checkpointing strategies at scale, complementary user studies are needed to validate its real-world applicability.

==> sections/Validation.tex <==
\input{Source/plots/fig/llm_e2e_time}

\section{Validation of the Experiment Design}
\label{sec:validation}

In this section, we aim to justify the validity of AI-agent-based experiment design. Specifically, we discuss the similarity between AI agents and human behavior in terms of code generation. We also explain why the experiment setting effectively measures the efficiency gain of notebook checkpointing from a causal perspective.

\paragraph{Similarity to Human Exploration Behavior}
Our decision to employ an AI agent for code generation and exploration is founded on recent research that demonstrates the capability of large language models (LLMs) to produce code (including data science code) and iterative refinement patterns that closely resemble those of human programmers~\cite{wei2022chain,hong2024data,guo2024ds, xu2022systematic}. Concretely, LLMs has been shown to:
\begin{enumerate}
\item \textbf{Generate high-quality data science code:} LLMs can generate high-quality code for data science tasks. For example, recent research shows LLM-based agent can achieve accuracy of 94.9\% on certain data analysis task benchmarks~\cite{hong2024data} and get mean ROC AUC performance of 0.82 on some feature engineering benchmarks~\cite{hollmann2024large}.

\item \textbf{Iteratively refine code:} Research in LLM agents~\cite{wei2022chain,yao2022react,shinn2024reflexion} shows that LLMs can parse feedback from external contexts to improve outputs. In our setup, the AI agent generates code step-by-step, receives execution feedback at each stage. Like a human data scientist, the AI agent can iteratively test, debug, and refine their work.
\end{enumerate}
While the AI agent is not subject to the same cognitive constraints as a human (e.g., short-term memory limitations or domain biases), these overlaps in behavior patterns provide reasonable assurance that our experimental tasks and the corresponding branching strategies align with real-world exploration scenarios. Moreover, as many data scientists use AI for coding assistance~\cite{nijkamp2022codegen, github_copilot,fried2022incoder}, their code may employ part of AI-agent-generated code.

\paragraph{Causal Perspective on Measuring Efficiency Gains}
A key rationale for our experiment is to measure, in a controlled manner, how much efficiency researchers can gain by using a notebook checkpointing mechanism (i.e.,\system). From a causal inference perspective, the central challenge is to isolate the effect of the checkpointing strategy from other factors, such as task difficulty or participants' skill level. Our design addresses this issue in two ways:

\begin{enumerate}
    \item \textbf{Consistency of Generated Code:} By using the same generated code across different checkpointing strategies, we ensure that our experiment holds task complexity and baseline code constant. Because the generated code and data do not change, any observed differences in runtime behavior or outcomes must stem from the checkpointing mechanism itself.
    
    \item \textbf{Consistency of Branching Strategy:} We introduce random selection to revisit previous cells, mirroring real-world data exploration where users backtrack to earlier steps~\cite{kery2018story,liu2019understanding}. Each branch emerges from the same generative process but differs in terms of whether it restarts the kernel, continues with the existing kernel state, or checks out a prior code-data version. This design ensures that all strategies face the same exploration tasks, allowing a fair comparison of performance.
\end{enumerate}

% reference papers:
% 1. AI-assistant data science code generation.\\
% - Github copilot (. For example, Codex [12]
% (the model used in Copilot), InCoder [24], and CodeGen [64] are GPT-style code generation models [68] trained on GitHub repositories (among other sources) that support code generation from texts and partial implementations in most mainstream programming)
% - Data Interpreter: An LLM Agent For Data Science (an LLM-based agent designed to automatically solve various data science problems end-to-end)
% - On the Design of AI-powered Code Assistants for Notebooks:
% 2. Similarity of the generated code between AI agent and human.\\
% - Evaluating large language models trained on code
% - A systematic evaluation of large language models of code
% - DATA INTERPRETER: AN LLM AGENT FOR DATA SCIENCE
% - Large Language Models for Automated Data Science: Introducing CAAFE for Context-Aware Automated Feature Engineering
% - DS-Agent: Automated Data Science by Empowering Large Language Models with Case-Based Reasoning
% 3. Similarity of the reasoning process between AI agent and human.\\
 % Goal: Why our AI agent-based experiment is valid? Randomized Controlled Trials? 

% Why AI is similar to human behavior in terms of code generation (quality)? cite some work stating the resemblance between human written code and AI-written code. Increasingly more people are adopting AI tools for writing their code, so they might be converging.  How to determine what to do next?

% Limitation: our rollback point is random.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

We overview notebook checkpointing frameworks (\cref{sec:background:checkpointing})
    and discuss the limitations of the existing evaluation (\cref{sec:existing_eval}).

\input{Source/plots/fig/fig_user_interface}

\subsection{Notebook Checkpointing}
\label{sec:background:checkpointing}

Computational notebooks (e.g., Jupyter, Colab) are designed around a linear, cell-by-cell execution model, even though real-world data science exploration is often iterative and non-linear. Practitioners commonly revisit older states, branch the code to try different alternatives, and switch among branches.~\cite{rule2018exploration,kery2019towards} To accommodate branching, they either start a new notebook for each path~\cite{chattopadhyay2020s} or mix branch-specific code cells in a single notebook~\cite{liu2019understanding,subramanian2019supporting,kery2018story}. Both approaches are time-consuming (re-running shared cells) and cognitively taxing (tracking which cells belong to each branch).

Inspired by code version control systems~\cite{gitbook}, \system~\cite{hanxichi}
% \footnote{\system is a work conditionally accepted as a paper by ACM CHI 2025.} 
addresses these issues by introducing \textbf{two-dimensional code+data checkpointing} for computational notebooks (see \cref{fig:ui:kishuboard} for its user interface). Unlike one-dimensional version control tools that track only code revisions, \system also version-controls the evolving “variable state in the kernel” or “data state” produced by each cell’s execution. Based on that, users can \textbf{checkout} the code and data state of notebook to any previous point and start exploring a new branch from that point. This feature, together with \system's UI that visualizes the branched structure of exploration similar to Git GUI~\cite{git_gui_clients}, enables fast, nonlinear data science exploration and reduces user's cognitive burden of managing multiple exploration branches simultaneously.



\subsection{Existing Evaluation of Notebook Checkpointing and its Limitations}
\label{sec:existing_eval}

The existing evaluation is based on human subject studies~\cite{hanxichi}. Specifically, to evaluate whether notebook checkpointing improves data science productivity, a user study was conducted with 20 student participants randomly split into experimental (with \system to checkout states) and control (without \system) groups. Both groups performed the same notebook-based tasks---building models, branching workflows, reporting metrics, retrieving previous variable states, debugging, and recovering from system crashes. While data practitioners may write their own code, participants in this study chose from a set of pre-written code snippets (with the option to modify them), ensuring that notebook checkpointing was the primary independent variable. The study measured each participant’s task completion time and gathered feedback through surveys, then compared performance between the two groups. 


Evaluation using traditional user study has several limitations:
\begin{enumerate}
  \item As it relies on a small group of participants, its statistical power is limited.
  % and making it challenging to observe a broad range of user behaviors.
    \item The short study duration restricts participants’ ability to engage in extended exploration. Even if they are allowed to branch and iterate, the limited time reduces opportunities to test multiple hypotheses or recover from mistakes.
    % that might occur in prolonged, real-world data analyses.
  \item The task steps and reference code snippets are provided, 
    limiting diverse exploration.
    % through more complex data science workflows.
\end{enumerate}

These limitations are inherent to  resource-constrained human-subject user study. 
To address them under the user-study paradigm, one would need to recruit more participants, extend the study duration, and ensure uniform expertise in data science and Python coding---all of which may involve substantial costs.
















==> sections/intro.tex <==


% S2: Background about KishuBoard

% S3: What we do: experiment design

% S3: Why Solid? 

% Goal: Why our AI agent-based experiment is valid? Randomized Controlled Trials? 

% Why AI is similar to human behavior in terms of code generation (quality)? cite some work stating the resemblance between human written code and AI-written code. Increasingly more people are adopting AI tools for writing their code, so they might be converging.  How to determine what to do next?

% Limitation: our rollback point is random.


\section{Introduction}

% S1: Introduction: 
% - our latest work
% - its limitation in empirical analysis
% - contribution: propose AI-agent-based evaluation in the context of KishuBoard, and also study KishuBoard.


Checkpointing computational notebooks can improve
    user productivity~\cite{hanxichi}.
Specifically, notebook systems like Jupyter~\cite{jupyter}, Colab~\cite{colab}, R Markdown~\cite{rmarkdown} let data scientists
    run a code block one at a time for
        analyzing tabular data, training machine learning models,
            visualizing results, etc.
By checkpointing intermediate code/data,
    users can undo undesirable executions,
        explore alternative hypotheses,
            and restore from crashes.
A recent work~\cite{hanxichi} proposes a checkpointing interface for computational notebooks
    and demonstrates its productivity benefits.

Unfortunately,
    the existing evaluation is limited to employing a handful of human subjects
        working on a fixed set of tasks.
While those participants are allowed
    to freely explore,
    the study remains constrained by the number of participants, 
        the variety of tasks, and the duration of the study.
We recognize that these limitations are inherent to 
    human subject studies: the limitations are difficult to overcome without adopting an entirely different approach.

In this work,
    we tackle them by devising an AI agent-based strategy.
Our observation is that AI agents can generate high-quality code akin to that produced by real data scientists, and exhibit iterative refinement behaviors that closely resemble the testing, debugging, and code improvement processes typically employed by human practitioners.
Specifically,
    we employ a pre-trained AI agent (i.e., ChatGPT 4o)
    to simulate real-world data scientists who explore data
        \textbf{with and without} a notebook checkpointing tool.
For each of the scenarios,
    the only independent variable is the assistance offered by the checkpointing tool;
    however, the actual variables residing in sessions
        and also elapsed times
        vary significantly.
%         because,
%     for example,
%         exploring an alternative hypothesis without checkpointing tools
%         may involve re-execution with variable renaming,
%             thus making the notebook significantly more \emph{messy}.
% Moreover,
%     re-executing code to restore a state can cause significant delays
%         when a large amount of data is involved.
% Our AI agent-based strategy naturally encompasses
%     these real-world complications
%         while considering hundreds of data exploration paths for variety.

This ``late-breaking work'', as a sequel to the recent research paper~\cite{hanxichi},
    expands the current state-of-the-art in two significant aspects.
First, we systematically evaluate the effectiveness of the new code+data space checkpointing framework
    with hundreds of data exploration scenarios. 
    % sampled from a modern generative language model (i.e., ChatGPT o1).
    This work is the first that evaluates data science checkpointing frameworks~\cite{li2023elasticnotebook,kishu,chex,wang2022diff}
        in such a large scale.
Second, we reason why our agent-based approach is valid,
    ensuring two types of consistencies:
        consistency of generated code and consistency of branching strategy.

